Alignist: CAD-Informed Orientation Distribution Estimation by Fusing Shape and Correspondences

Object pose distribution estimation is crucial in robotics for better path planning and handling of symmetric objects. Recent distribution estimation approaches employ contrastive learning-based approaches by maximizing the likelihood of a single pose estimate in the absence of a CAD model. We propose a pose distribution estimation method leveraging symmetry respecting correspondence distributions and shape information obtained using a CAD model. Contrastive learning-based approaches require an exhaustive amount of training images from different viewpoints to learn the distribution properly, which is not possible in realistic scenarios. Instead, we propose a pipeline that can leverage correspondence distributions and shape information from the CAD model, which are later used to learn pose distributions. Besides, having access to pose distribution based on correspondences before learning pose distributions conditioned on images, can help formulate the loss between distributions. The prior knowledge of distribution also helps the network to focus on getting sharper modes instead. With the CAD prior, our approach converges much faster and learns distribution better by focusing on learning sharper distribution near all the valid modes, unlike contrastive approaches, which focus on a single mode at a time. We achieve benchmark results on SYMSOL-I and T-Less datasets.

==> sec/6_Limitations.tex <==
\section{Limitations and Future Work}
Our approach doesn't explicitly utilize the texture cues from the image or the CAD model. Instead, it utilizes the features from SurfEmb which depend on both texture and geometry simultaneously. Employing another expert that models the texture cues explicitly will enable us to model distribution which would help us handle objects like SphereX on Symsol-II where the shape expert cannot contribute towards the distribution.     
